Measurement Schemes for Quantum Linear Equation Solvers

Solving Computational Fluid Dynamics (CFD) problems requires the inversion of a linear system of equations, which can be done using a quantum algorithm for matrix inversion arxiv:1806.01838. However, the number of shots required to measure the output of the system can be prohibitive and remove any advantage obtained by quantum computing. In this work we propose a scheme for measuring the output of QSVT matrix inversion algorithms specifically for the CFD use case. We use a Quantum Signal Processing (QSP) based amplitude estimation algorithm arxiv:2207.08628 and show how it can be combined with the QSVT matrix inversion algorithm. We perform a detailed resource estimation of the amount of computational resources required for a single iteration of amplitude estimation, and compare the costs of amplitude estimation with the cost of not doing amplitude estimation and measuring the whole wavefunction. We also propose a measurement scheme to reduce the number of amplitudes measured in the CFD example by focusing on large amplitudes only. We simulate the whole CFD loop, finding that thus measuring only a small number of the total amplitudes in the output vector still results in an acceptable level of overall error.

==> nozzle_table.tex <==
\begin{tblr}{colspec={p{1.45cm}p{1.6cm}p{1.6cm}p{1.45cm}p{1.45cm}p{1.45cm}p{1.45cm}p{1.45cm}},
row{odd}={bg=lightgray},
row{1}={bg=white}}
No. Stations & Compressible & Coupled & Converged $\epsilon_{\textrm{max}}$ & \% of Converged with $\epsilon > \epsilon_{\textrm{tol}}$ & Max Error / $\epsilon_{\textrm{tol}}$ & Converged $\alpha_{\textrm{min}}$ & $\alpha_{\textrm{min}}$ of $\epsilon > \epsilon_{\textrm{tol}}$ \\
\hline 
8 & False & False & $1\times 10^{-8}$ & 6.25 & $8.96\times 10^{6}$ & 0.25 & 0.25 \\
8 & False & True & $1\times 10^{-8}$ & 6.25 & $3.55\times 10^{9}$ & 0.25 & 0.25 \\
8 & True & False & $5\times 10^{-8}$ & 10.94 & $1.22\times 10^{6}$ & 0.25 & 0.25 \\
8 & True & True & $1\times 10^{-4}$ & 31.37 & $5.66\times 10^{6}$ & 0.25 & 0.50 \\
16 & False & False & $1\times 10^{-8}$ & 25.00 & - & 0.25 & 0.25 \\
16 & False & True & $1\times 10^{-8}$ & 7.84 & $2.01\times 10^{8}$ & 0.25 & 0.25 \\
16 & True & False & $5\times 10^{-8}$ & 9.38 & $1.53\times 10^{6}$ & 0.25 & 0.25 \\
16 & True & True & $1\times 10^{-5}$ & 15.69 & $7.45\times 10^{5}$ & 0.25 & 0.75 \\
\end{tblr}

